Gaussian processes at the Helm(holtz): A more fluid model for ocean currents

Given sparse observations of buoy velocities, oceanographers are interested in reconstructing ocean currents away from the buoys and identifying divergences in a current vector field. As a first and modular step, we focus on the time-stationary case - for instance, by restricting to short time periods. Since we expect current velocity to be a continuous but highly non-linear function of spatial location, Gaussian processes (GPs) offer an attractive model. But we show that applying a GP with a standard stationary kernel directly to buoy data can struggle at both current reconstruction and divergence identification, due to some physically unrealistic prior assumptions. To better reflect known physical properties of currents, we propose to instead put a standard stationary kernel on the divergence and curl-free components of a vector field obtained through a Helmholtz decomposition. We show that, because this decomposition relates to the original vector field just via mixed partial derivatives, we can still perform inference given the original data with only a small constant multiple of additional computational expense. We illustrate the benefits of our method with theory and experiments on synthetic and real ocean data.

==> ICML_2023_-_GP_Oceans/sections/1introduction.tex <==
Ocean currents are key to the global distribution of water, heat, and nutrients. To better understand ocean currents, scientists are interested in two tasks: (1) ocean current prediction and (2) identification of divergences, also known as upwellings and downwellings, in the current vector field.
Predicting ocean currents accurately can facilitate weather forecasting, maritime navigation, and forecasting of oil spill dispersion.
And current divergences are important to identify since they are responsible for the transport of biomass, carbon, and nutrients -- with implications for ecosystem management, climate, and the fishing industry \citep{dasaro2018ocean}. %,Huguenard2016OnTN,Androulidakis2018InfluenceOR
With these tasks in mind, researchers release and track GPS-tagged buoys in the ocean \citep{ozgokmen2012carthe,dasaroLASERdata2017}.

It remains to choose an appropriate method to reconstruct currents and their divergences from the buoy data. \citet{goncalves2019naive} and \citet{lodise2020investigating} proposed modeling buoy velocities in the latitude and longitude directions according to independent Gaussian processes (GPs) with standard spatiotemporal kernels (e.g., squared exponential kernels). In our work, we focus on the spatial aspects of this task and assume the velocity field is stationary in time. Even under this simplification, an independent spatial GP prior on the velocities is a natural choice due to its ability to handle the sparsity of buoy observations on the ocean surface and its assumption that currents vary smoothly but in a highly nonlinear fashion. We call this model the \emph{velocity GP}.

% A spatial GP prior on the velocities is a natural choice due to its ability to handle the sparsity of buoy observations on the ocean surface and its assumption that currents vary smoothly but in a highly nonlinear fashion. \textcolor{red}{DRB:mention stationarity somewhere in intro}

However, in what follows, we show that there remains substantial room for improvement. In simulated cases where we have access to ground truth, we observe that the velocity GP approach can fail to complete vortices or fail to connect currents when buoys are observed sparsely. And while we show how to derive divergence estimates for the velocity GP, we also find that these estimates often fail to capture the true divergence when it is known in simulations or real data.

To address these shortcomings, we propose to instead model more directly known behaviors from fluid dynamics.
In particular, scientists know that the motion of a volume element of a continuous fluid medium in two dimensions consists of (i) expansion or contraction in two orthogonal directions, (ii) rotation about an instantaneous axis, and (iii) translation. A \emph{Helmholtz decomposition} \citep{bhatia2013helmoltzhodge, arfken1999mathematical} from fluid dynamics lets us decompose the vector field of ocean currents into a \emph{divergent} component (or \emph{curl-free}, measuring expansion, contraction, and translation) and a \emph{rotational} component (or \emph{divergence-free}, measuring rotation).\footnote{The \emph{divergent component} is also called \emph{curl-free} because applying  the curl operator to this component gives the function that is zero everywhere. Similarly, the \emph{rotational component} is also called \emph{divergence-free} because the divergence of this component is zero everywhere. See \cref{prop:div-curl-free} for more details.}

By contrast to the standard approach, we model the divergent and rotational components with independent GP priors, rather than the velocity components. Our resulting \emph{Helmholtz GP} prior offers several conceptual advantages. For one, oceanographers expect the two components to have substantially different magnitudes and length scales; it is straightforward to encode these differences with a Helmholtz GP. By contrast, we prove that the velocity GP forces a shared magnitude across divergent and rotational components. Second, we expect correlation between the longitudinal and latitudinal components of a current, which the Helmholtz GP exhibits -- and the velocity GP lacks by construction. Finally, the Helmholtz GP is agnostic to the (arbitrary) choice of reference frame, while the velocity GP is not.

We demonstrate that our Helmholtz GP is amenable to practical inference. Since (i) the Helmholtz decomposition is based on partial (mixed) derivatives, and (ii) the derivative of a GP is a GP, we show that our prior choice implies a GP prior on the current itself. Therefore, we can still perform inference given the original data with no extra approximation. And our method suffers no increase in computational complexity relative to the velocity GP.

Finally, we demonstrate the superior performance of our Helmholtz GP at the current prediction task and divergence estimation task (as well as vorticity estimation) in a variety of simulated and real experiments. Code is available at \url{https://github.com/renatoberlinghieri/Helmholtz-GP}.
 
\textbf{Related work.} The Helmholtz decomposition has been used extensively in the oceanographic literature as a way to interpret and visualize currents' features when the field is observed on a grid \citep{rocha2016mesoscale, zhang2018helm1, zhang2019helm3, lei2020helm2, buhler2014wave, caballero2020integration}. These works decompose the observed vector field in the two Helmholtz components, but do not solve any prediction task. Recent studies also demonstrate a direct dynamical significance of the different Helmholtz components on the flow of energy across spatiotemporal scales in the ocean; the rotational component is found to transfer energy from small scales to larger while the divergent component is key to transferring energy to smaller scales where energy is dissipated \citep{contreras2022understanding, srinivasan2023forward}. In the GP literature, it is well known that specific covariance functions can be used to capture curl- and divergence-free vector fields \citep{alvarez2012kernels, fuselier2007refined, lowitzsch2002approximation}; moreover, a line of research related to electromagnetism \citep{wahlstrom2013modeling, wahlstrom2015modeling, solin2018modeling} uses curl- and divergence-free kernels to try to reconstruct the overall magnetization through Maxwell's equations, similarly to what we are doing for ocean currents. However, none of the aforementioned work can be directly applied to our setting, either because the observation model is different, or because curl- and divergence-free fields are not considered together, as we do with the Helmholtz decomposition. Finally, recent work from the deep learning community \citep{greydanus2022dissipative} extended Hamiltonian Neural Networks \citep{greydanus2019hamiltonian} to model both curl- and divergence-free dynamics simultaneously. Although the prediction problem is similar, the authors test this method only on low-resolution data available on a dense grid. We show results of this method for (sparse) buoy data in \cref{sec:experiments} and \cref{app:experiment}, where we find that it often produces physically implausible predictions. We discuss related work further in \cref{app:related_work}. 



==> ICML_2023_-_GP_Oceans/sections/2background.tex <==
% \documentclass[../main.tex]{subfiles}
% \graphicspath{{\subfix{../images/}}}
% \begin{document}
\section{Background}\label{sec:background}

In what follows, we first describe the problem setup. Then we establish necessary notation and concepts from the Helmholtz decomposition and Gaussian processes.

\textbf{Problem Statement.} %\label{sec:background-problem} 
We consider a dataset $D$ of $M$ observations, $\{(\bfx_m, \bfy_m)\}_{m=1}^M$. Here $\bfx_m = (x_m^{(1)}, x_m^{(2)})^\top \in \R^2$ represents the location of a buoy, typically a longitude and latitude pair. We treat $\bfx_m$ as a column vector. And $\bfy_m = (y_m^{(1)}, y_m^{(2)})^\top \in \R^2$ gives the corresponding longitudinal and latitudinal velocities of the buoy (the so-called drifter trace). For $m \in \{1, \ldots, M\}$, we consider $\bfy_m$ as a sparse noisy observation of a 2-dimensional vector field, $F : \R^2 \rightarrow \R^2$, mapping spatial locations into longitudinal and latitudinal velocities, $F(\bfx_m) = (F^{(1)}(\bfx_m), F^{(2)}(\bfx_m))^\top$. We assume that the velocity field is stationary in time, and so $F$ is not a function of time. Our primary goals are (1) prediction of the field $F$ at new locations, not observed in the training data, and (2) estimation of the divergence, itself a function of location and which we define next as part of the Helmholtz decomposition. Secondarily, we are interested in recovering vorticity, another functional of $F$ described below.

\textbf{The Helmholtz Decomposition.} The motion of a volume element of a fluid, such as the ocean, can be decomposed into a divergent velocity and a rotational velocity. 
\begin{definition}[Helmholtz decomposition, {{\citealp{bhatia2013helmoltzhodge}}}]
\label{th:helmdec}
A twice continuously differentiable and compactly supported vector field $F : \mathbb{R}^2 \rightarrow \mathbb{R}^2$ can be expressed as the sum of the gradient of a scalar potential $\Phi: \R^2 \to\R$, called the \textit{potential function}, and the vorticity operator of another scalar potential $\Psi: \R^2 \to \R$, called the \textit{stream function}:
\begin{align}
\underbrace{F (\bfx)}_{\text{ocean flow}} = \underbrace{\mathrm{grad} \,\Phi(\bfx)}_{\text{divergent velocity}} + \underbrace{\mathrm{rot}\, \Psi(\bfx)}_{\text{rotational velocity}}
\end{align}
where $\bfx = (x^{(1)}, x^{(2)})^\top$, and
\begin{align}
\mathrm{grad} \,\Phi(\bfx) \!\coloneqq\!
\begin{bmatrix}
\partial\Phi(\bfx)/\partial x^{(1)} \\ \partial\Phi(\bfx)/\partial x^{(2)}
\end{bmatrix} \, \text{and} \,
\mathrm{rot}\,\Psi(\bfx) \!\coloneqq\!
\begin{bmatrix}
\partial\Psi(\bfx)/\partial x^{(2)} \\
-\partial\Psi(\bfx)/\partial x^{(1)}
\end{bmatrix}.
\end{align}
\end{definition}

The \emph{divergence} of $F$ (denoted $\delta$) and the \emph{vorticity} of $F$ (denoted $\zeta$) at a point $\bfx$ are
\begin{align}
\label{eqn:divergence-standard}
\delta(\bfx) &\!\coloneqq\!
\mathrm{div}(F(\bfx)) \!\coloneqq\!
\frac{\partial F^{(1)}(\bfx)}{\partial x^{(1)}} +        \frac{\partial F^{(2)}(\bfx)}{\partial x^{(2)}}
=\frac{\partial^2\Phi(\bfx)}{\partial^2 x^{(1)}} + \frac{\partial^2\Phi(\bfx)}{\partial^2 x^{(2)}}
 \\
%
\label{eqn:vorticity-standard}
\zeta(\bfx) &\!\coloneqq\!
\mathrm{curl}(F(\bfx))\!\coloneqq\!
\frac{\partial F^{(1)}(\bfx)}{\partial x^{(2)}} - \frac{\partial F^{(2)}(\bfx)}{\partial x^{(1)}}
\!=\frac{\partial^2\Psi(\bfx)}{\partial^2 x^{(2)}} + \frac{\partial^2\Psi(\bfx)}{\partial^2 x^{(1)}}. 
\end{align}

In \cref{eqn:divergence-standard}, $\mathrm{div}(F)$ depends only on $\Phi$ because $\mathrm{div}  (\mathrm{rot}\,\Psi ) = 0$. In other words, the rotational velocity is divergence-free. Similarly, in \cref{eqn:vorticity-standard}, $\mathrm{curl}(F)$ depends only on $\Psi$ because $\mathrm{curl} (\mathrm{grad} \,\Phi ))=0$. In other words, the divergent velocity is curl-free. We review the $\mathrm{grad}$, $\mathrm{rot}$, $\mathrm{div}$, and $\mathrm{curl}$ operators -- and explore the equations above in more detail -- in \cref{app:divcurl}. We summarize the various terms in \cref{tab:relationships}. In \cref{app:helmholtz}, we present a graphical illustration of a Helmholtz decomposition of a selected vector field, and we further discuss the importance of divergence and vorticity within ocean currents.

% Here we are implicitly using the fact that the divergence of the vorticity component is zero,


% as well as the $\text{curl}$ of the divergence component,

% \textcolor{red}{(RG: I have opinions about the $\nabla \times$ notation that I want to make a placeholder for to remind myself to think / talk about.  In short, it's nice / standard to think of $\nabla$ as a vector of partial derivative operators, but then you need to be more careful that your curl and dot products make formal sense.)}
% so that then to get $\delta$ and $\zeta$ it is enough to apply the two operators to the corresponding components. Note that 

\begin{table}[t]
\caption{Terms and notation around the divergence and vorticity.}
\label{tab:relationships}
\begin{center}
\begin{tabular}{c | c}
$\Phi$ & potential function \\
$\mathrm{grad}\,\Phi$ & divergent velocity \\
%$\nabla \Phi$ & divergent velocity \\

$\delta = \mathrm{div} (\mathrm{grad} \,\Phi)$ & divergence \\ \hline
$\Psi$ & stream function \\ 
$\mathrm{rot}\,\Psi$ & rotational velocity \\ 
$\zeta = \mathrm{curl}(\mathrm{rot} \,\Psi)$ & vorticity
\end{tabular}
\end{center}
\end{table}



\textbf{Bayesian Approach and Gaussian Process Prior.} %\label{sec:background-gps}
In what follows, we will take a Bayesian approach to inferring $F$. In particular, we assume a likelihood, or noise model, relating the observed buoy velocities to the field $F$:
\begin{align}\label{eqn:likelihood}
\bfy_m = F(\bfx_m) + \bfeps_m, \quad \bfeps_m  \stackrel{\text{ind}}{\sim} \mathcal{N}(0, \obsvar\mathbf{I}_2), \quad 1 \leq m \leq M,
\end{align}
for some $\obsvar>0$ and independent ($\stackrel{\text{ind}}{\sim}$) noise across observations. Here and throughout, we use $\mathbf{I}_p \in R^{p \times p}$ to denote the identity matrix in $p$ dimensions. We use $0$ to denote the zero element in any vector space.


Before defining our prior, we review Gaussian processes (GPs). Let $\bfx, \bfx'\in \featurespace$ represent two input vectors. Assume that we want to model a $P$-dimensional function $G: \featurespace \to \R^P$, $G(\bfx) = (G^{(1)}(\bfx), \dotsc, G^{(P)}(\bfx))^\top$.  A $P$-output GP on covariate space $\featurespace$ is determined by a mean function $\mu : \featurespace \to \R^P$, $\mu(\bfx) = (\mu^{(1)}(\bfx), \dotsc, \mu^{(P)}(\bfx))^\top$, and a positive definite kernel function $k : \featurespace \times \featurespace \to \R^{P \times P}$. We use $k(\bfx, \bfx')_{i, j}$ to denote the $(i,j)$th output of $k(\bfx, \bfx')$. We say that $G$ is GP distributed and write $G\sim \mathcal{GP}(\mu, k)$ if for any $N \in \mathbb{N}$, for any $(\bfx_1, \dotsc, \bfx_N) \in \R^{2 \times N}$, and for any vector of indices $(p_1, \dotsc, p_N) \in \{1, \dotsc, P\}^N$, $(G^{(p_n)}(\bfx_n))_{n=1}^N$ is an $N$-dimensional Gaussian random variable with mean vector $(\mu^{(p_n)}(\bfx_n))_{n=1}^N$ and covariance matrix with $(i, j)$th entry $k(\bfx_i, \bfx_j)_{p_i, p_j}$. See \citet{alvarez2012kernels} for a review of multi-output GPs.

% Before defining our prior, we review Gaussian processes. A Gaussian process on a covariate space $\featurespace$ is determined by a mean function $\mu : \featurespace \to \R$ and a positive definite kernel function $k : \featurespace \times \featurespace \to \mathbb{R}$. Consider two sequences of points $\bfZ = (\bfz_1,\ldots,\bfz_M) \in \featurespace^M$ and $\bfZ' = (\bfz'_1,\ldots,\bfz'_{M'}) \in \featurespace^{M'}$ with $\bfz_m, \bfz'_{m'} \in \featurespace$. Let $k(\bfZ,\bfZ')$ denote the $M \times M'$ matrix with $k(\bfZ,\bfZ')_{m,m'} = k(\bfz_m, \bfz_{m'})$.
% Let $f: \featurespace \to \R$ denote a generic function, and let $f(\bfZ)$ denote $(f(\bfz_1), \ldots, f(\bfz_M))^\top$. Then we say $f \sim \GP(\mu,k)$ if $f$ is marginally Gaussian at any finite set of locations with $f(\bfZ) \sim \normal(\mu(\bfZ), k(\bfZ,\bfZ))$.

%While Gaussian processes can be extended to a function with two-dimensional output like $F: \R^2 \to \R^2$, the setup can become complex.
% To describe a vector-field $F$ with outputs in $\R^2$ rather than $\R$ using Gaussian processes,
% we augment the domain of $F$ to include an index defining the output dimension. 
% Define $\gamma: (\R^2 \times \{1,2\}\to\R)\to (\R^2 \to \R^2)$ by $(\gamma(G)(a,b))^{(i)} = G(a,b,i)$ for all $(a,b,i) \in \R^{2} \times \{1,2\}$. 
% $\gamma$ is a linear bijection.
% We therefore equivalently define $\tilde{F} = \gamma^{-1}(F)$ such that for any $(\dt{x}{1}, \dt{x}{2}),\ \tilde{F}(\dt{x}{1}, \dt{x}{2}, i)=F(\dt{x}{1},\dt{x}{2})^{(i)}$ and take $\tilde{F} \sim \GP(\mu,k)$ as our prior. It remains to choose $\mu$ and $k$.
% write $F^{(j_m)}(\bfx_m) = \tilde{F}(\bfx_m^{(1)}, \bfx_m^{(2)}, j_m)$ for a function $\tilde{F}: \R^2 \times \{1,2\} \to \R$, with input vector $\bfz_m = (\bfx_m^{(1)}, \bfx_m^{(2)}, j_m)^\top$. 

\textbf{Velocity Gaussian Process.} In spatial data analysis, commonly $\mu$ is chosen to be identically 0. And a conventional choice for $k$ would be an isotropic kernel\footnote{We say a kernel $k$ is isotropic if there exists some $\kappa: \R^+\rightarrow \R$ such that for any $\bfx$ and $\bfx'$ in $\R^2,\ k(\bfx, \bfx')=\kappa(\|\bfx-\bfx'\|).$} separately in each output dimension. That is, for any $\bfx, \bfx' \in \featurespace$,
\begin{align}
	% k_{\text{SE}}(\bfx, \bfx')_{i,j} =  \mathbf{1}_{\{i=j\}} \sigma^2_{F_j} \exp\left(-\frac{\|\bfx -  \bfx'\|_2^2}{2\ell_j^2}\right). 
 	k_{\text{vel}}(\bfx, \bfx')=  \begin{bmatrix} k^{(1)}(\bfx, \bfx') & 0 \\
  0 & k^{(2)}(\bfx, \bfx') 
  \end{bmatrix}.
  \label{eqn:vel-kernel}
\end{align}
where $k^{(1)}$ and $k^{(2)}$ are isotropic kernels. We call this choice the \emph{velocity GP} to emphasize that the independent priors are directly on the observed velocities. A standard isotropic kernel choice for $k^{(i)}$, $i \in \{1,2\}$, is the squared exponential kernel,
\begin{align}\label{eqn:sq-exp-kernel} 
k_{\text{SE}}^{(i)}(\bfx, \bfx') = \sigma^2_{i} \exp\left(-\tfrac{1}{2}\|\bfx -  \bfx'\|_2^2/\ell_i^2\right).
\end{align}

The velocity GP with squared exponential kernels for each component (henceforth, the \emph{\sevelgp}) has four hyperparameters: for $i \in \{1,2\}$, the signal variance $\sigma^2_i > 0$ determines the variation of function values from their mean in the $i$th output dimension, and $\ell_i > 0$ controls the length scale on which the function varies. 

% We extend the definition of the mean and kernel function to allow for arbitrary finite collections of inputs. In particular, for $\mathbf{X}=(\bfx_1, \dotsc, \bfx_N) \in \R^{2 \times N}$ and $\mathbf{X'}=(\bfx'_1, \dotsc, \bfx'_{N'}) \in \R^{2 \times N}$,

% \begin{align}
%     \mu(\mathbf{X}) = 
%     \begin{pmatrix}
%         \mu^{(1)}(\mathbf{X}) \\ \mu^{(2)}(\mathbf{X})
%     \end{pmatrix}
%     \quad \text{and} \quad 
%     k(\mathbf{X}, \mathbf{X'}) = 
%     \begin{pmatrix}
%         k(\mathbf{X}, \mathbf{X'})_{1,1} & k(\mathbf{X}, \mathbf{X'})_{1,2} \\ 
%         k(\mathbf{X}, \mathbf{X'})_{2,1} & k(\mathbf{X}, \mathbf{X'})_{2,2}
%     \end{pmatrix}
% \end{align}
% where (a) for $i \in \{1,2\}$, $n \in \{1,\ldots,N\}$, $\mu^{(i)} (\mathbf{X})$ is an $N$-dimensional vector with $n$th entry $\mu_i (\bfx_n)$, and (b) for $i,j \in \{1,2\}$, $n \in \{1,\ldots,N\}$, $n' \in \{1,\ldots,N'\}$, $k(\mathbf{X},\mathbf{X'})_{i,j}$ is an $N \times N'$ matrix with $(n, n')$th entry $k(\bfx_n,\bfx'_{n'})_{i,j}$. See \cite{alvarez2012kernels} for a complete analysis of multi-output GPs.

==> ICML_2023_-_GP_Oceans/sections/3method.tex <==
% \documentclass[../main.tex]{subfiles}
% \graphicspath{{\subfix{../images/}}}
% \begin{document}

% Consider a dataset of M observations, $\{\textbf{x}_m, \textbf{y}_m\}_{m=1}^M$, where $\textbf{x}_m =  (x_m^{(1)}, x_m^{(2)})$ represents the spatial location of a buoy, and $\textbf{y}_m = (\text{y}_m^{(1)}, \text{y}_m^{(2)})$ the corresponding horizontal and vertical velocities (the so-called drifter trace). We treat these $\textbf{y}$'s as sparse noisy observations of a 2D vector field, $\text{F} : \mathbb{R}^2 \rightarrow \mathbb{R}^2$, mapping spatial locations into horizontal and vertical velocities, $(\text{F}^{(1)}, \text{F}^{(2)})$.
%
% We model the drifter traces as follows, with observation noise $\sigma^2_{\text{obs}}$:
% \begin{equation}
% \begin{bmatrix}
% \text{y}_m^{(1)} \\ \text{y}_m^{(2)}
% \end{bmatrix} \mid \text{F}(\textbf{x}_m) \stackrel{\text{ind}}{\sim} \mathcal{N}\left(\text{F}(\textbf{x}_m), \begin{bmatrix}
% \sigma^2_{\text{obs}} & 0 \\ 0 & \sigma^2_{\text{obs}}
% \end{bmatrix} \right)
% \label{eqn:likelihood}
% \end{equation}

% independently across $m$.

Instead of putting separate GP priors with isotropic kernels on the two components of $F$ as in the velocity GP, we propose to put separate GP priors with isotropic kernels on the Helmholtz scalar potentials $\Phi$ and $\Psi$. In this section, we describe our model and how to retrieve the quantities of interest from it. In the next section, we describe its conceptual strengths over the velocity GP, which we see empirically in \cref{sec:experiments}.

\textbf{Our Helmholtz GP prior.} To form our new \emph{Helmholtz GP} prior, we put independent GP priors on the Helmholtz stream and potential functions:
\begin{equation}
\label{eqn:helmprior}
 \Phi \sim \GP(0, k_{\Phi}) \quad \text{and} \quad
    \Psi \sim \GP(0, k_{\Psi}), 
\end{equation} 
where we take $k_{\Phi}$ and $k_{\Psi}$ to be isotropic kernels. When these kernels are chosen to be squared exponentials (\cref{eqn:sq-exp-kernel}), we call our model the \emph{\sehelmgp}. The $\sehelmgp$ has four parameters: $\ell_{\Phi}$ and $\sigma^2_{\Phi}$ for $k_{\Phi}$, and $\ell_{\Psi}$ and $\sigma^2_{\Psi}$ for $k_{\Psi}$. In principle we could use any two kernels such that sample paths of the resulting GPs are almost surely continuously differentiable. Generally, we will want to be able to consider divergences and vorticities of the implied process, which will require sample paths of the implied process to be at least twice-continuously differentiable. For the latter condition to hold, it is sufficient for $k_{\Phi}(0, \bfx)$ and $k_{\Psi}(0, \bfx)$ to have continuous mixed partial derivatives up to order five; see \citet[Theorem 2.09 \& Section 7.2]{lindgren2012stationary}.


First, we check that our prior yields a GP prior over the vector field $F$.

\begin{restatable}{proposition}{helmprior}\label{prop:helm-prior}
%    Let $F$ be the ocean current vector field and $\Phi$ and $\Psi$ the potential and stream functions of a Helmholtz decomposition of the field, respectively.
Let $F$ be an ocean current vector field defined by potential and stream functions that are a priori independent and distributed as 
$\Phi \sim \GP(0, k_{\Phi})$ and 
$\Psi \sim \GP(0, k_{\Psi})$, where $k_{\Phi}$ and $k_{\Psi}$ are such that $\Phi$ and $\Psi$ have almost surely continuously differentiable sample paths.
Then
%\begin{align}
% \Phi \sim \GP(0, k_{\Phi}) \hspace{5pt}
%\end{align}
%Then
\begin{align}
F = \mathrm{grad} \,\Phi + \mathrm{rot}\, \Psi \sim \GP(0, \khelm ),
\end{align}
where, for $\bfx, \bfx'\in \featurespace$, 
\begin{align}
\khelm(\bfx, \bfx') = 
{
\renewcommand*{\arraystretch}{3.5}
\begin{bmatrix}
\dfrac{
        \partial^2 k_{\Phi}(\bfx, \bfx')
    }{
        \partial x^{(1)} \partial (x')^{ {(1)}}
    }
    +
    \dfrac{
        \partial^2 k_{\Psi}(\bfx, \bfx')
    }{
        \partial x^{(2)} \partial (x')^{ {(2)}}
    } &\ \ \ \ 
\dfrac{
        \partial^2 k_{\Phi}(\bfx, \bfx')
    }{
        \partial x^{(1)} \partial (x')^{ {(2)}}
    }
    -
    \dfrac{
        \partial^2 k_{\Psi}(\bfx, \bfx')
    }{
        \partial x^{(2)} \partial (x')^{ {(1)}}
    }  \\ 
\dfrac{
        \partial^2 k_{\Phi}(\bfx, \bfx')
    }{
        \partial x^{(2)} \partial (x')^{ {(1)}}
    }
    -
    \dfrac{
        \partial^2 k_{\Psi}(\bfx, \bfx')
    }{
        \partial x^{(1)} \partial (x')^{ {(2)}}
    }  &\ \ \ \ 
\dfrac{
        \partial^2 k_{\Phi}(\bfx, \bfx')
    }{
        \partial x^{(2)} \partial (x')^{ {(2)}}
    }
    +
    \dfrac{
        \partial^2 k_{\Psi}(\bfx, \bfx')
    }{
        \partial x^{(1)} \partial (x')^{ {(1)}}
    }   
\end{bmatrix}.
}
\end{align}
\end{restatable}
% \begin{remark}
% \Cref{prop:helm-prior} holds more generally, so long as the kernel has continuous mixed partial derivatives up to order two.
% \end{remark}
Our proof in \cref{app:prior-helm-gp} relies on two observations: (i) the Helmholtz decomposition is based on partial (mixed) derivatives and (ii) the derivative of a GP is a GP; see, e.g., \citet[Chapter 9.4]{rasmussen2005gp}, and \citet[Theorem 2.2.2]{adler1981geometry}.

\textbf{Making predictions.}
To make predictions using our Helmholtz GP, we need to choose the hyperparameter values and then evaluate the posterior distribution of the ocean current given those hyperparameters.

We choose the GP hyperparameters by maximizing the log marginal likelihood of the training data.
To write that marginal likelihood, we let $\Xtrain \in \R^{2 \times M}$ be the matrix with $m$th column equal to $\bfx_m$.
We define $\Ytrain = (\bfy_1^{(1)}, \ldots, \bfy_M^{(1)},\bfy_1^{(2)}, \ldots, \bfy_M^{(2)})^\top \in \R^{2M}$. We extend the definition of the mean and kernel function to allow for arbitrary finite collections of inputs. In particular, for $\mathbf{X}=(\bfx_1, \dotsc, \bfx_N) \in \R^{2 \times N}$ and $\mathbf{X'}=(\bfx'_1, \dotsc, \bfx'_{N'}) \in \R^{2 \times N'}$,

\begin{align}
    \mu(\mathbf{X}) = 
    \begin{pmatrix}
        \mu^{(1)}(\mathbf{X}) \\ \mu^{(2)}(\mathbf{X})
    \end{pmatrix}
    \quad \text{and} \quad 
    k(\mathbf{X}, \mathbf{X'}) = 
    \begin{pmatrix}
        k(\mathbf{X}, \mathbf{X'})_{1,1} & k(\mathbf{X}, \mathbf{X'})_{1,2} \\ 
        k(\mathbf{X}, \mathbf{X'})_{2,1} & k(\mathbf{X}, \mathbf{X'})_{2,2}
    \end{pmatrix}
\end{align}
where (a) for $i \in \{1,2\}$, $n \in \{1,\ldots,N\}$, $\mu^{(i)} (\mathbf{X})$ is an $N$-dimensional column vector with $n$th entry $\mu^{(i)} (\bfx_n)$, and (b) for $i,j \in \{1,2\}$, $n \in \{1,\ldots,N\}$, $n' \in \{1,\ldots,N'\}$, $k(\mathbf{X},\mathbf{X'})_{i,j}$ is an $N \times N'$ matrix with $(n, n')$th entry $k(\bfx_n,\bfx'_{n'})_{i,j}$. With this notation, we denote the covariance of the training data with itself, under the full model including noise, as $\Khtrtr = k(\Xtrain,\Xtrain) + \obsvar \mathbf{I}_{2M}$. Then the log marginal likelihood is 
\begin{align}
\label{eqn:log-marginal-likelihood}
\begin{split}
\log p(\Ytrain \mid \Xtrain)&= \log \mathcal{N}(\Ytrain; 0, \Khtrtr) \\ 
    &=-\frac{1}{2} \Ytrain^T \Khtrtr^{-1}\Ytrain - \frac{1}{2} \log |\Khtrtr| - \frac{2M}{2} \log 2\pi,
\end{split}
\end{align}
where $|\cdot |$ takes the determinant of its matrix argument.
We provide details of our optimization procedure in \cref{sec:experiments}.

With hyperparameter values in hand, we form probabilistic predictions using the posterior of the GP. In particular, the posterior mean forms our prediction at a new set of points, and the posterior covariance encapsulates our uncertainty.

Consider $N$ new (test) locations at which we would like to predict the current. We gather them in $\Xtest \in \R^{2 \times N}$, with $n$th column equal to $\bfx_n^\star$. We denote the covariance of various training and testing combinations as:
$\Khtetr = k(\Xtest,\Xtrain)$ and
$\Khtete = k(\Xtest,\Xtest)$.
Then a posteriori after observing the training data $D$, the $2N$-long vector $(F^{(1)}(\bfx_1^\star), \dotsc,F^{(1)}(\bfx_N^\star),\dotsc,F^{(2)}(\bfx_1^\star)\dotsc, F^{(2)}(\bfx_N^\star))^\top$ describing the current at the test locations has a normal distribution with mean
\begin{equation}\label{eqn:helm_posterior_mean}
    \mu_{F \mid D} = \Khtetr \Khtrtr^{-1} \Ytrain
\end{equation}
and covariance
\begin{equation}\label{eqn:helm_posterior_cov}
    K_{F \mid D} = \Khtete - \Khtetr \Khtrtr^{-1} \Khtetr^\top.
\end{equation}

For more details, see \citet[Section 2.2]{rasmussen2005gp}. Note that these formulas can be used to evaluate posterior moments of the velocity field for either the Helmholtz GP (setting $k = \khelm$) or the velocity GP (with $k = \kvel$). 


\textbf{Recovering divergence and vorticity.} We next show how to recover the posterior distributions on the divergence and vorticity scalar fields given a posterior on the current field $F$. We can estimate divergence and vorticity at any location by using the posterior mean at that point, and we can report uncertainty with the posterior variance. Note that our formulas recover divergence and vorticity for either our Helmholtz GP or the velocity GP. 

\begin{restatable}{proposition}{divergenceofagp}
\label{prop:divergenceofagp}
Let $F \sim \mathcal{GP}(\mu, k)$ be a two-output Gaussian process with almost surely continuously differentiable sample paths. Then, for $\bfx, \bfx'\in \featurespace$, 
\begin{align}
&\delta = \mathrm{div} \, F \sim \mathcal{GP}(\mathrm{div} \, \mu, k^{\delta}) \\ %\quad \text{and} \\
&\zeta = \mathrm{curl} \, F \sim \mathcal{GP}(\mathrm{curl} \, \mu, k^{\zeta})
\end{align}
where
%
% k_{\textup{div}}
\begin{align}
 &k^{\delta}(\bfx, \bfx') = \!\!\!\!\!\sum_{(i,j) \in \{1, 2\}^2} \!\!\!\!\!\frac{\partial^2 k(\bfx,\bfx')_{i,j}}{\partial x^{(i)}\partial x^{(j)}}
\\ %\quad \text{and} \\
&k^{\zeta}(\bfx, \bfx') \!=\!\!\!\!\! \sum_{(i,j) \in \{1, 2\}^2}\!\!\!\! (-1)^{i+j}\frac{\partial^2 k(\bfx, \bfx')_{i,j}}{\partial x^{(3-i)}\partial x^{(3-j)}}.
\end{align}
\end{restatable}

We provide the proof for \cref{prop:divergenceofagp} in \cref{app:div-vort-gp}.

% \begin{restatable}{proposition}{posteriordivergencehelmholtz}
% Let $\tilde{F}$ be the ocean current vector field, modeled by a GP prior with mean $0$ and kernel function $k_{\text{Helm}}$ as in \cref{prop:helm-prior}. Assuming the likelihood model in \cref{eqn:likelihood}, the divergence and vorticity conditional on the data are GPs as well, \textcolor{red}{DRB:todo, define tilde divergences}
% \begin{align*}
% \label{eqn:postdiv}
%  \tilde{\delta} \mid D \sim \text{GP}(\mu_{\delta \mid D}, k_{\delta \mid D}) \\ 
%   \tilde{\zeta} \mid D \sim \text{GP}(\mu_{\zeta \mid D}, k_{\zeta \mid D})
% \end{align*}
% with $\mu_{\delta \mid D}, K_{\delta \mid D}, \mu_{\zeta \mid D}, K_{\zeta \mid D}$ as in \cref{app:postdivergence}.
% \end{restatable}

\textbf{Computational Cost.} Since the latitude and longitude outputs are correlated under the Helmholtz GP, it generally has a higher computational cost than the velocity GP. We establish that the extra cost should be no worse than a small constant factor.

\begin{proposition}
\label{prop:comp-cost}
    Take $M$ training data points. Let $C_{vel}(M)$ and $C_{helm}(M)$ be the computational costs for evaluating the log marginal likelihood (\cref{eqn:log-marginal-likelihood}) via Cholesky factorization or QR decomposition for the velocity GP and Helmholtz GP, respectively. Then 
    \begin{equation*}
        \lim_{M \rightarrow \infty} C_{helm}(M)/C_{vel}(M) \leq 4
    \end{equation*}
\end{proposition}

The cost of computing the log marginal likelihood is dominated by the cost of solving the linear system $\Khtrtr^{-1}\Ytrain$ and computing the log determinant $|\Khtrtr|$. Both of these costs in turn arise primarily from the cost of computing a factorization of $\Khtrtr$. Let $\mathrm{CF}(s)$ be the cost of factorizing a square matrix with $s$ rows with Cholesky or QR factorization. Due to the two (correlated) current outputs, the cost of the Helmholtz GP is dominated by $\mathrm{CF}(2M)$. In the velocity GP, the two outputs are uncorrelated and can be handled separately, so the cost is dominated by $2 \mathrm{CF}(M)$. Therefore, $\lim_{M \rightarrow \infty} C_{helm}(M) / C_{vel}(M)\leq \mathrm{CF}(2M)/ (2 \mathrm{CF}(M))$. Since the cost of the Cholesky and QR factorization algorithms is a polynomial with degree at most 3, the result follows. 

In \cref{app:comp-cost} we provide similar computational results for the task of prediction and also discuss some nuances of how any of these results may change in the presence of special structure.
%computational costs further, by deriving a similar cost bound for the computation of Helmholtz posteriors at new test locations.




==> ICML_2023_-_GP_Oceans/sections/4methodadvantages.tex <==

We next describe three key advantages of the Helmholtz GP prior over the velocity GP prior: (1) more physically realistic prior assumptions reflecting the relative magnitude and length scales of the divergence and vorticity, (2) more physically realistic correlation of the longitudinal and latitudinal velocities of current at any point, and (3) equivariance to reference frame.

\textbf{Prior magnitude of the divergence and vorticity.} In real ocean flows, the divergence is known a priori to have both a substantively different magnitude and different length scale relative to the vorticity. In what follows, we argue that the Helmholtz GP is able
to capture the relative contributions of divergence and vorticity directly in the prior -- whereas the velocity GP does not have this direct control.


%We first discuss the magnitude point here% and then turn to the length scale point below.
On the magnitude side, the divergence is known to contribute much less to the current than the vorticity contributes.
%In a perfect two-dimensional flow, the divergence is exactly zero.
%Non-zero divergence at the surface of the real ocean is observed only because ocean flow is slightly three-dimensional.  However, the ocean is much wider than it is deep, and so the divergence is typically of smaller order than the vorticity. \textcolor{red}{DRB: Is the width relative to depth really the reason we expect more divergence than vorticity? I don't see how this immediately follows, so would like a bit of clarification if so.}
If we consider a SE Helmholtz GP, the signal variance hyperparameters $\sigma_\Phi^2$ and $\sigma_\Psi^2$ control the magnitude of $\Phi$ and $\Psi$;
as a direct consequence of the linearity of the divergence $\delta$ and vorticity $\zeta$ in $\Phi$ and $\Psi$ (\Cref{eqn:divergence-standard,eqn:vorticity-standard}), the marginal variances of $\delta$ and $\zeta$ scale linearly with $\sigma_\Phi^2$ and $\sigma_\Psi^2$, respectively. The model can therefore directly and separately control the magnitude of the rotational and divergence components. A similar argument can be applied to more general Helmholtz GPs with parameters controlling the magnitude of $\Phi$ and $\Psi$.

%Moreover, we see from the result just below that the induced Helmholtz GP kernels on the divergence and vorticity will in turn have the output magnitude controlled by these signal variances.
%
%\begin{proposition} \label{prop:helmholtz_gp_magnitude}
%Let $\Phi \sim \GP(0,k_{\Phi})$ and $\Psi \sim \GP(0,k_{\Psi})$. Let $\khelm^\delta$ and $\khelm^\zeta$ be the induced Helmholtz GP kernels on the divergence and vorticity. \textcolor{red}{TB: refer to some earlier results/equations} Then $\khelm^\delta$ results from a linear operator applied to $k_{\Phi}$ and has no dependence on $k_{\Psi}$. Likewise, $\khelm^\zeta$ results from a linear operator applied to $k_{\Psi}$ and has no dependence on $k_{\Phi}$. 
%\end{proposition}



%\begin{proposition} \label{prop:vel_gp_magnitude}
%Let $F^{(1)} \sim \GP(0,k^{(1)})$ and $F^{(2)} \sim \GP(0,k^{(2)})$. Let $\kvel^\delta$ and $\kvel^\zeta$ be the induced Helmholtz GP kernels on the divergence and vorticity. \textcolor{red}{TB: refer to some earlier results/equations} Then both $\kvel^\delta$ and $\kvel^\zeta$ result from linear operators with nontrivial dependence on both $k^{(1)}$ and $k^{(2)}$.
%\end{proposition}
% \setcounter{footnote}{\value{footnote}+1}

%\footnotetext[\value{footnote}]{We say a kernel $k$ is isotropic if there exists some $\kappa: \R^+\rightarrow \R$ such that for any $\bfx$ and $\bfx'$ in $\R^2,\ k(\bfx, \bfx')=\kappa(\|\bfx-\bfx'\|).$  For example, squared exponential kernels are isotropic.}

By contrast, the velocity GP provides no such control.
In fact, for any isotropic choice of $k^{(1)}$ and $k^{(2)}$ we show that the resulting velocity GP must assume the same variance on the divergence and vorticity in the prior.
%   As described above, this assumption is inappropriate for ocean currents.

\begin{restatable}{proposition}{propEqualVarDivVort}\label{prop:equal-var-div-vort}
Let $k^{(1)}$ and $k^{(2)}$ be isotropic kernels with inputs $\bfx, \bfx' \in \R^2$. Take $F^{(1)} \sim \mathcal{GP}(0, k^{(1)})$ and $F^{(2)}\sim \mathcal{GP}(0, k^{(2)})$ independent. Suppose  $k^{(1)}$ and $k^{(2)}$ are such that $F^{(1)}, F^{(2)}$ have almost surely continuously differentiable sample paths.
Let $\delta$ and $\zeta$ be defined as in \cref{eqn:divergence-standard,eqn:vorticity-standard}.
Then for any $\bfx,\mathrm{Var}[\delta(\bfx)] = \mathrm{Var}[\zeta(\bfx)]$.
\end{restatable}
The proof of \cref{prop:equal-var-div-vort} appears in \cref{app:sec-equal-marginal-var}.


\textbf{Prior length scales of the divergence and vorticity.} The divergence and vorticity are also known to operate
on very different length scales in real ocean flows.  Vorticity operates over long length scales, whereas divergence tends to be more localized. Similarly to the argument above, the Helmholtz GP allows control over the length scale in each of its components, which directly control the length scale of the divergence and vorticity. 
In particular, if $k_\Phi(\bfx, \bfx') = \kappa(\|\bfx-\bfx'\|/\ell)$, for some $\kappa:\R^+\rightarrow \R,$ then $k^{\delta}(\bfx, \bfx') = \ell^{-4}\eta(\|\bfx-\bfx'\|/\ell)$ for another function $\eta:\R^+\rightarrow \R$ that does not depend on $\ell$; see \Cref{sec:appendix_length_scale_relationship}.
By contrast, the velocity GP requires setting the length scales of its priors in tandem, and it is unclear how to control the length scales of the divergence and vorticity.


\textbf{Correlations between longitudinal and latitudinal current components.} Ocean flows have correlation between longitudinal and latitudinal velocities at single locations and across different locations.   For instance, within a vortex, the longitudinal velocity at six o'clock (relative to the center of the vortex) coincides with a zero latitudinal velocity at that same location, and also with a non-zero latitudinal velocity at three o'clock. Likewise, the occurrence of divergence at a given point induces a latitudinal velocity at six o'clock (with no longitudinal velocity), as well as a non-zero longitudinal velocity at three o'clock (with no latitudinal velocity).  By modeling the divergence and vorticity directly, the Helmholtz prior induces 
correlation between the longitudinal and latitudinal components,
which is absent in the velocity GP prior. 

%It is important to observe that in this study, the behavior at a single point is considered in the context of small neighborhoods around those points. This is necessary to allow us to talk about correlations between collections of vectors.


\textbf{Equivariance to reference frame.}
We now show the Helmholtz GP is agnostic to the choice of reference frame defined by longitude and latitude, but the velocity GP is not.

\begin{restatable}{proposition}{propEquivariance}\label{prop:Equivariance}
%Let $\Phi \sim \GP(0,k_{\Phi})$ and $\Psi \sim \GP(0,k_{\Psi})$ for any isotropic $k_{\Phi}$ and $k_{\Psi}$.
Let $\mu_{F \mid D}(\Xtest, \Xtrain, \Ytrain)$ denote the Helmholtz GP posterior mean for training data $\Xtrain, \Ytrain$ and test coordinates $\Xtest$,
and let $R$ be an operator rotating coordinates and velocities about $(0,0)$.
Then 
\begin{equation}\label{eqn:helm_equivariance}
\!\!\!\mu_{F\mid D}(R\Xtest, R\Xtrain, R\Ytrain) \!=\! R\mu_{F\mid D}(\Xtest, \Xtrain, \Ytrain).
\end{equation}
\end{restatable}

\Cref{prop:Equivariance} formalizes that it is equivalent to either (1) rotate the data and then predict using the Helmholtz GP or (2) predict using the Helmholtz GP and rotate the prediction. The proof of \cref{prop:Equivariance} is given in \cref{app:equivariancehelmgp}.


\begin{remark}
The equivariance property in \cref{prop:Equivariance} need not hold for velocity GP priors. Consider the following counterexample. Let $F^{(1)} \sim \GP(0,k^{(1)})$ for some nontrivial isotropic $k^{(1)}$. And $F^{(2)} = 0$, a trivial isotropic prior.
Take any data $\Xtrain$, $\Ytrain$, $\Xtest$, and a positive (counterclockwise) $90^{\circ}$ rotation. 
Due to the trivial prior in the second coordinate, the posterior in the second coordinate has mean $\mu^{(2)}_{F\mid D}(\Xtest, \Xtrain, \Ytrain) = 0$.
If we rotate the data first, the posterior in the second coordinate is still zero, and generally the posterior in the first coordinate will be nontrivial.
Conversely, if we first compute the posterior and then rotate the mean, the posterior in the first coordinate will now be zero instead, and the posterior in the second coordinate will be nonzero.
Therefore, the equality in \cref{eqn:helm_equivariance} does not hold for this velocity GP.
\end{remark}

% %%%%%%%%%%%%%%%%%
\input{sections/mse_table.tex}
%%%%%%%%%%%%%%%%%%%%%

==> ICML_2023_-_GP_Oceans/sections/5experiment.tex <==
% \documentclass[../main.tex]{subfiles}
% \graphicspath{{\subfix{../images/}}}
% \begin{document}


We next empirically compare the $\sehelmgp$ and $\sevelgp$. We show that the $\sehelmgp$ yields better current predictions as well as better divergence (and vorticity) identification, across a variety of simulated and real data sets, compared to the $\sevelgp$ and a neural network approach.

\textbf{Data.} In our experiments, we use only the spatial locations of buoys and discard time; that is, for now we make the simplifying assumption that currents are stationary across time to focus our comparison of the $\sehelmgp$ and $\sevelgp$. We leave incorporation of time to future work.

The real datasets we use consist of drifter traces of GPS-tagged buoys in the ocean. While oceanographers have some knowledge that allows a rough assessment of the real data, only in simulations we do have access to ground truth currents, divergences, and vorticities. Therefore, we run a variety of simulations with current vector fields reflecting known common ocean behaviors. We simulate buoy trajectories by initializing buoys at a starting point and allowing the current field to drive their motion. See \cref{app:experiment} for more details of our setup in each specific simulation.

\textbf{Baselines.} We focus on comparing our $\sehelmgp$ to the $\sevelgp$. In \cref{app:experiment} and \cref{tab:mse}, we also compare with dissipative Hamiltonian neural networks (D-HNNs) by \citet{greydanus2022dissipative}. Generally we find worse performance for D-HNNs compared to either GP method.

In what follows, we emphasize visual comparisons both because the distinctions between methods are generally clear and because it is illuminating to visually pick out behaviors of interest. We also provide root mean squared error (RMSE) comparisons in \cref{tab:mse}. However, we note that the RMSE can be expected to vary as one changes either the ocean area or the densities (or more generally locations) of test points, and both of these choices must always be somewhat arbitrary. % For the purposes of \cref{tab:mse}, we choose the test points to lie on a rectangular grid that is somewhat larger than the training data.

\textbf{Algorithmic details.} In our comparisons, each full model including an $\sehelmgp$ prior or an $\sevelgp$ prior has five hyperparameters: $\sigma^2_{\Phi}$, $\ell_{\Phi}$, $\sigma^2_{\Psi}$, $\ell_{\Psi}$, $\obsvar$ and $\ell_1, \sigmaFu^2, \ell_{2}, \sigmaFv^2, \obsvar$, respectively. In each case, we fit the log of the hyperparameters by maximizing the marginal likelihood using Adam \citep{kingma2015adam}. We optimize in the log-scale and then exponentiate the optimal values to ensure positivity of the hyperparameters. We run each experiment until the log marginal likelihood changes by less than $10^{-4}$, which occurs in fewer than 2000 iterations for all experiments. With the exception of the GLAD data (which presents special difficulties that we describe in \cref{app:experiments-glad}), we found that results were not sensitive to initialization. To train the D-HNN, we ran the code from \citet{greydanus2022dissipative}. More algorithmic details are provided individually for each experiment in \cref{app:experiment}.

\subsection{Simulated experiments}

We focus on simulations of key ocean behaviors of interest to oceanographers: vortices, concentrated divergences, and combinations thereof. As a summary across simulation experiments in \cref{tab:mse}, we see that -- for predictions, divergence estimates, and vorticity estimates -- the $\sehelmgp$ is most accurate by RMSE on a majority of tasks, often by a substantial factor. We next examine individual experiments more closely; all simulated experiments are described in detail in \cref{app:sec-synthetic-experiments}. 

\begin{figure*}[t]
    \centering
    \includegraphics[trim={0 0.25cm 0 0.08cm},clip, draft=False, width=\textwidth]{images/vortex_main.pdf}
    \caption{First column: ground truth predictions (upper) and divergence (lower). Second column: current predictions. Third column: divergence estimates. Fourth column: posterior divergence z-values.}
    \label{fig:vortex}
\end{figure*}


\textbf{Vortex with zero divergence.} First, we consider a single vortex with no divergence. The $\sehelmgp$ is better at predicting the current and identifying the lack of divergence.

In a vortex, water particles rotate around a central point. The black arrows in the upper left plot of \cref{fig:vortex} show the ground-truth vector field at test points, with longitude on the horizontal axis and latitude on the vertical axis. Red arrows show our simulated buoy trajectories, which we give to all methods as training data. See \cref{app:subsectionvortex} for additional details of the setup and results. 

The second column shows predictions from the $\sehelmgp$ (upper) and $\sevelgp$ (lower) at the test points. The red arrows are still the training data. Despite having access only to data from one side of the vortex, the $\sehelmgp$ is able to reconstruct the full vortex. The $\sevelgp$ is not. 

The ground truth divergence is identically 0 throughout the domain and depicted in the lower left plot. The third column shows divergence estimates from the $\sehelmgp$ (upper) and $\sevelgp$ (lower) on the same color scale. The fourth column helps us understand if either posterior is reporting a nonzero divergence. In particular, for each point we plot a ``z-value'': precisely, the posterior mean at that point divided by the posterior standard deviation. One might, for instance, conclude that a method has detected a nonzero divergence if the magnitude of the z-value is greater than 1.
From the third column, we conclude that the $\sehelmgp$ estimate of the divergence is closer to the ground truth of zero than the $\sevelgp$. From the fourth column, we see that neither method concludes nonzero divergence, but the $\sehelmgp$ posterior is more concentrated near zero.

\textbf{Vortex adjacent to a straight current.}
In \cref{app:sec-vortex-current}, we consider a vortex adjacent to a current that runs across the bottom of our view. The ground truth divergence is zero. The $\sehelmgp$ correctly estimates no divergence. The $\sevelgp$ erroneously and very confidently reports a divergence -- with z-values reaching above 6 in magnitude.

\textbf{Duffing oscillator with areas of concentrated divergence.} We next simulate a classic example called a Duffing oscillator, and we add two areas of divergence; the ground truth current appears in the upper left plot of \cref{fig:duffing}, and the ground truth divergence appears in the lower left. The simulated buoy trajectories appear in red. See \cref{app:sec-duffing-divergence} for further details on setup and results.

We see in the second column that the $\sehelmgp$ (upper) is largely able to reconstruct the two vortices in the Duffing oscillator (upper left), though it struggles with the upper right current. By contrast, the $\sevelgp$ is not able to connect the currents continuously across the two sides of the space, in disagreement with conservation of momentum. 

Again, the third column depicts divergence estimates from both methods, and the fourth column depicts z-values. In this case, both methods accurately recover the two areas of divergence. In \cref{app:sec-duffing-divergence,fig:smallduffing,fig:midduffing,fig:bigduffing}, we experiment with smaller and larger areas of divergence with the Duffing oscillator. In \cref{app:sec-divergence}, we isolate areas of divergence without the Duffing oscillator. Across the six experiments involving regions of divergence, the $\sehelmgp$ typically outperforms the $\sevelgp$ in detecting these regions -- often by a substantial margin, as shown in \cref{tab:mse}. In these same experiments, the $\sehelmgp$ similarly outperforms the $\sevelgp$ at predicting the velocity field.

\textbf{A note on vorticity.} Although we have not focused on vorticity estimation in the main text, we report it for each of our experiments in \cref{app:experiment}. Generally we see superior performance for vorticity estimation from the $\sehelmgp$ relative to the $\sevelgp$, similar to divergence estimation. The RMSEs in \cref{tab:mse} are always better for the $\sehelmgp$, except for one experiment. And the visual comparisons for each experiment in \cref{app:experiment} confirm this finding. For example, the $\sehelmgp$ is very good in predicting zero vorticity when there is no vorticity, whereas the $\sevelgp$ fails in this task (\cref{fig:smalldivapp,fig:middivapp,fig:bigdivapp}).


\begin{figure*}[t]
    \centering
    \includegraphics[trim={0 0.24cm 0 0.06cm}, clip, width=\textwidth]{images/duffing_divsmall_main.pdf}
    \caption{First column: ground truth predictions (upper) and divergence (lower). Second column: current predictions. Third column: divergence estimates. Fourth column: posterior divergence z-values.}
    \label{fig:duffing}
\end{figure*}


\subsection{Real-data experiments}

Although ground truth currents and divergences are not available for real data, we can still assess performance against oceanographers' expert knowledge.

\textbf{LASER data.} The LAgrangian Submesoscale ExpeRiment \citep{dasaroLASERdata2017} was performed in the Gulf of Mexico in 2016. The full dataset spans two winter months and more than 1000 buoys; see \cref{app:experiments-laser} for details. We focus on a particular spatial area and 2-hour time span in which oceanographers expect to see a particular convergent front. Moreover, restricting the time span makes a stationarity assumption more appropriate. We are left with 19 buoys. When recorded spatial coordinates overlap across data points, we observe that both the $\sehelmgp$ and the $\sevelgp$ treat all data as noise. While this issue merits further investigation and model development, for now we downsample across time to form the final data sets here.


The left column of \cref{fig:laser} shows the current predictions using the $\sehelmgp$ (upper) and $\sevelgp$ (lower). Red arrows show the observed buoy data, with 55 total observations across all buoys. The black arrows show the current posterior means at test locations. In this case, the two sets of predictions are qualitatively very similar.

The second column shows the divergence predictions for the $\sehelmgp$ (upper) and $\sevelgp$ (lower); the third column shows the z-values for the respective posterior distributions. The $\sehelmgp$ predicts a negative divergence area (light blue diagonal) that agrees with the spatial region where oceanographers expect a convergent front. By contrast, the $\sevelgp$ does not identify any divergence. 

\begin{figure*}[t]
    \centering
    \includegraphics[trim={0 0.25cm 0 0.06cm},clip,width=\textwidth]{images/lasersparse_main.pdf}
    \caption{First column: current predictions. Second column: divergence estimates. Third column: posterior divergence z-values.}
    \label{fig:laser}
\end{figure*}

We find that the discrepancy between the $\sehelmgp$ and the $\sevelgp$ observed in \cref{fig:laser} depends on the amount of data. When we double the amount of data from that in \cref{fig:laser} (by downsampling less), we find that both methods are able to recover the same convergent front; see \cref{app:experiments-laser,fig:laserfull}. This finding then also corroborates that the convergent front in fact does exist and looks like the posterior detection by the $\sehelmgp$ in \cref{fig:laser}. In that way, the finding further lends support to the superior performance of the $\sehelmgp$ in \cref{fig:laser}.



\textbf{GLAD data.} The Grand Lagrangian Deployment (GLAD) experiment \citep{ozgokmen2012carthe} was conducted  near the Deepwater Horizon site and Louisiana coast in July 2012. The full dataset consists of over 300 buoys. Unlike the winter LASER data, the summer GLAD data faces additional challenges from regular oscillations due to wind (rather than current); see \cref{app:experiments-glad} for more details. Rather than account for these oscillations, for the moment we ameliorate their effect by downsampling considerably both in time and across buoys. We are left with 85 observations.

The current predictions between the $\sehelmgp$ and $\sevelgp$ are generally quite similar (\cref{fig:gladsparse,fig:gladfull}). Although in this case we do not have any ground truth from oceanographers in advance, some features of the $\sehelmgp$ prediction seem more realistic from physical intuition: namely, the downturn in the lower left region of the plot and the vortex in the upper left region of the plot. We also note that the $\sehelmgp$ and $\sevelgp$ predict substantially different divergences: respectively, zero and nonzero.

To check that our $\sehelmgp$ method is computationally reasonable, we run on a larger subset of the GLAD data with 1200 data points. We find that it takes less than 10 minutes to optimize the hyperparameters, form predictions, and estimate the divergences at the test points. 



% \end{document}

==> ICML_2023_-_GP_Oceans/sections/6discussion.tex <==
% \documentclass[../main.tex]{subfiles}
% \graphicspath{{\subfix{../images/}}}
% \begin{document}

We have demonstrated the conceptual and empirical advantages of our Helmholtz GP relative to the velocity GP. A number of challenges remain. While we have focused on the purely spatial case for modularity, in general we expect currents to change over time, and it remains to extend our method to the spatiotemporal case -- which we believe should be straightforward. Moreover, \citet{goncalves2019naive,lodise2020investigating} used more complex kernels with two length scales per dimension in their spatiotemporal extension of the velocity GP. From known ocean dynamics, we expect that in fact two length scales would be appropriate in the Helmholtz GP for modeling the vorticity -- but unnecessary for the divergence.
While our independent Gaussian noise model is standard in spatiotemporal modeling -- and shared by \citet{goncalves2019naive,lodise2020investigating} -- our real-data experimentation suggests that a better noise model might account for short-term wind oscillations and other noise patterns distinctive to oceans.



==> ICML_2023_-_GP_Oceans/sections/mse_table.tex <==
\begin{table*}[t]
\vskip 0.15in
\caption{Green identifies the lowest RMSE. Dark green indicates the RMSE is at least two times smaller than the next best model.}
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{c|| c | c| c|| c| c| c || c| c | c}
& \multicolumn{3}{c ||}{Velocity $F$} & \multicolumn{3}{c||}{Divergence $\delta$} & \multicolumn{3}{c}{Vorticity $\zeta$} \\
\toprule
 & \makecell{Helm} & \makecell{Vel} & \makecell{D-hnn} & \makecell{Helm} &  \makecell{Vel} & \makecell{D-hnn} & \makecell{Helm}   & \makecell{Vel} 
   & \makecell{D-hnn} \\
%\midrule
\hline \hline
\makecell{vortex} & \darkcell0.24 & 0.72 & 0.54 & \darkcell0.0 & 0.22 & 0.87 & \lightcell0.77 & 1.05 & 1.03 \\ \hline
\makecell{vortex w/ straight current} & 0.30 & 0.49 & \lightcell0.28 & \darkcell0.0 & 0.57 & 0.51& \lightcell0.88   & 1.08& 1.91 \\ \hline
\makecell{small divergence} & 1.11 & 1.25 & \lightcell0.67 & 2.62 & \lightcell1.45  & 4.14 & \darkcell0.0  & 1.07 & 0.31 \\ \hline
\makecell{medium divergence} & \lightcell0.17 & 0.19 & 0.55 & 0.39 & \lightcell0.33 & 1.32 & \darkcell0.05 & 0.12 &  0.38\\ \hline
\makecell{big divergence} & \darkcell0.04 & 0.10 & 0.19 & \lightcell0.05 & 0.12 & 0.27 & \darkcell0.00 & 0.10 & 0.11  \\ \hline
\makecell{duffing w/ small divergence} & \darkcell0.96 & 2.05 & 2.14 & \lightcell0.94 & 0.95 & 1.89 & \lightcell1.40 & 2.28 & 2.64 \\ \hline
\makecell{duffing w/ medium divergence} & \darkcell0.19 & 0.60 & 1.65 & \darkcell0.14 & 0.50 & 1.15 & \lightcell0.24 & 0.26 & 2.39 \\ \hline
\makecell{duffing w/ big divergence} & 0.41 & \lightcell0.22 & 1.63 & \darkcell0.08 & 0.17 & 1.10 & 0.48 & \darkcell0.16 & 2.41 \\ \hline
\bottomrule
%\hline \hline
%\makecell{vortex} & \darkcell0.0556 & 0.5138 & 0.2948 & \darkcell0.0 & 0.0488 & 0.7531 & \lightcell0.5553 & 1.0999 & 1.0520 \\ \hline
%\makecell{continuous current \\ w/ vortex} & 0.0906 & 0.2422 & \lightcell0.0761 & \darkcell0.0 & 0.3204 & 0.2615& \lightcell0.7697   & 1.1620   & 3.6360 \\ \hline
%\makecell{small divergence} & 1.2263 & 1.5851 & \lightcell0.4531 & 6.8784 & \darkcell2.1250  & 17.1530 & \darkcell0.0  & 1.1537 & 0.0987 \\ \hline
%\makecell{medium divergence} & \lightcell0.0280 & 0.0344 & 0.3017 & 0.1519 & \lightcell0.1063 & 1.7428 & \darkcell0.0029 & 0.0141 &  0.1426\\ \hline
%\makecell{big divergence} & \darkcell0.0020 & 0.0108 & 0.0357 & \lightcell0.0028 & 0.0155 & 0.0717 & \darkcell0.0 & 0.0106 & 0.0113  \\ \hline
%\makecell{duffing w/ \\ small divergence} & \darkcell0.9236 & 4.2070 & 4.5906 & \lightcell0.8815 & 0.9199 & 3.5554 & \lightcell1.9602 & 5.1951 & 6.9440 \\ \hline
%\makecell{duffing w/ \\ medium divergence} & \darkcell0.0832 & 0.3629 & 2.7370 & \darkcell0.0183 & 0.2500 & 1.3161 & 0.2738 & \darkcell0.0655 & 5.7267 \\ \hline
%\makecell{duffing w/ \\ big divergence} & 0.2028 & \lightcell0.0511 & 2.6441 & \darkcell0.0065 & 0.0282 & 1.2195 & 0.2884 & \darkcell0.0261 & 5.8246 \\ \hline
%\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\label{tab:mse}
\end{table*}
